Meta-learning from Learning Curves Challenge: Lessons learned from the First Round and Design of the Second Round

Meta-learning from learning curves is an important yet often neglected research area in the Machine Learning community. We introduce a series of Reinforcement Learning-based meta-learning challenges, in which an agent searches for the best suited algorithm for a given dataset, based on feedback of learning curves from the environment. The first round attracted participants both from academia and industry. This paper analyzes the results of the first round (accepted to the competition program of WCCI 2022), to draw insights into what makes a meta-learner successful at learning from learning curves. With the lessons learned from the first round and the feedback from the participants, we have designed the second round of our challenge with a new protocol and a new meta-dataset. The second round of our challenge is accepted at the AutoML-Conf 2022 and currently ongoing .

==> backup-table-2nd-round.tex <==
\begin{tabular}{|c|lc|ccccc|} 
\hline
\textbf{PHASE}                                                         & \multicolumn{2}{c|}{\textbf{DATASET}}                                               & \textbf{\textbf{DDQN}}                  & \textbf{BOS}  & \textbf{FT}   & \textbf{\textbf{AR}}   & \textbf{RS}    \\ 
\hline
\multirow{15}{*}{\begin{tabular}[c]{@{}c@{}}Development \\phase\end{tabular}} & 0  & \textcolor[rgb]{0.075,0.075,0.075}{ADULT}\textcolor[rgb]{0.075,0.075,0.075}{}  & 0.74                                    & \textbf{0.75} & \textbf{0.75} & 0.72                   & 0.16           \\
                                                                       & 1  & \textcolor[rgb]{0.075,0.075,0.075}{CADATA}\textcolor[rgb]{0.075,0.075,0.075}{} & 0.64                                    & 0.62          & 0.64          & \textbf{\textbf{0.72}} & 0.52           \\
                                                                       & 2  & \textcolor[rgb]{0.075,0.075,0.075}{DIGITS}\textcolor[rgb]{0.075,0.075,0.075}{} & 0.64                                    & 0.73          & 0.73          & \textbf{\textbf{0.74}} & 0.25           \\
                                                                       & 3  & \textcolor[rgb]{0.075,0.075,0.075}{DOROTHEA~}                                  & 0.62                                    & 0.65          & 0.63          & 0.6                    & \textbf{0.67}  \\
                                                                       & 4  & NEWSGROUPS                                                                     & 0.06                                    & 0.11          & 0.11          & \textbf{\textbf{0.15}} & 0.13           \\
                                                                       & 5  & CHRISTINE                                                                      & \textbf{\textbf{0.39}}                  & 0.37          & 0.36          & 0.32                   & 0.3            \\
                                                                       & 6  & JASMINE                                                                        & \textbf{\textbf{0.56}}                  & \textbf{0.56} & \textbf{0.56} & 0.54                   & \textbf{0.56}  \\
                                                                       & 7  & MADELINE                                                                       & \textbf{\textbf{\textbf{\textbf{0.5}}}} & 0.43          & 0.37          & 0.4                    & 0.4            \\
                                                                       & 8  & PHILIPPINE                                                                     & \textbf{\textbf{0.39}}                  & 0.36          & 0.36          & 0.25                   & 0.33           \\
                                                                       & 9  & SYLVINE                                                                        & \textbf{\textbf{0.86}}                  & 0.85          & 0.84          & 0.79                   & 0.84           \\
                                                                       & 10 & ALBERT                                                                         & \textbf{\textbf{0.26}}                  & 0.21          & 0.21          & 0.17                   & 0.21           \\
                                                                       & 11 & DILBERT                                                                        & \textbf{\textbf{0.66}}                  & 0.47          & 0.47          & 0.37                   & 0.28           \\
                                                                       & 12 & FABERT                                                                         & \textbf{\textbf{0.25}}                  & 0.24          & 0.2           & 0.17                   & 0.22           \\
                                                                       & 13 & ROBERT                                                                         & \textbf{\textbf{0.22}}                  & 0.16          & 0.16          & 0.12                   & 0.0            \\
                                                                       & 14 & VOLKERT                                                                        & \textbf{\textbf{0.13}}                  & 0.11          & 0.11          & 0.0                    & 0.12           \\ 
\hline
\multirow{15}{*}{\begin{tabular}[c]{@{}c@{}}Final\\phase\end{tabular}} & 15 & ALEXIS                                                                         & 0.21                                    & \textbf{0.5}  & \textbf{0.5}  & 0.1                    & 0.0            \\
                                                                       & 16 & DIONIS                                                                         & 0.17                                    & 0.28          & 0.28          & \textbf{\textbf{0.44}} & 0.18           \\
                                                                       & 17 & GRIGORIS                                                                       & 0.0                                     & \textbf{0.39} & \textbf{0.39} & 0.03                   & 0.0            \\
                                                                       & 18 & JANNIS                                                                         & 0.31                                    & \textbf{0.32} & \textbf{0.32} & 0.17                   & \textbf{0.32}  \\
                                                                       & 19 & WALLIS                                                                         & \textbf{\textbf{0.42}}                  & 0.24          & 0.24          & 0.16                   & 0.31           \\
                                                                       & 20 & EVITA                                                                          & \textbf{\textbf{0.54}}                  & 0.5           & 0.47          & 0.36                   & 0.53           \\
                                                                       & 21 & FLORA                                                                          & \textbf{\textbf{0.48}}                  & 0.13          & 0.13          & 0.14                   & 0.47           \\
                                                                       & 22 & HELENA                                                                         & 0.06                                    & 0.11          & 0.11          & 0.1                    & \textbf{0.12}  \\
                                                                       & 23 & TANIA                                                                          & \textbf{\textbf{0.48}}                  & 0.17          & 0.17          & 0.0                    & 0.0            \\
                                                                       & 24 & YOLANDA                                                                        & -0.01                                   & \textbf{0.12} & \textbf{0.12} & -0.15                  & 0.0            \\
                                                                       & 25 & ARTURO                                                                         & 0.52                                    & 0.62          & 0.61          & 0.43                   & \textbf{0.67}  \\
                                                                       & 26 & CARLO                                                                          & -0.03                                   & -0.13         & -0.13         & -0.3                   & \textbf{0.0}   \\
                                                                       & 27 & \textcolor[rgb]{0.075,0.075,0.075}{MARCO~}                                     & 0.54                                    & \textbf{0.6}  & \textbf{0.6}  & 0.25                   & 0.56           \\
                                                                       & 28 & PABLO                                                                          & \textbf{\textbf{0.24}}                  & \textbf{0.24} & \textbf{0.24} & \textbf{\textbf{0.24}} & 0.0            \\
                                                                       & 29 & WALDO                                                                          & \textbf{\textbf{0.41}}                  & 0.39          & 0.39          & 0.34                   & 0.16           \\ 
\hline
\rowcolor[rgb]{0.949,0.949,0.949} \multicolumn{3}{|c|}{\textbf{AVERAGE }}                                                                                    & \textbf{\textbf{0.38}}                  & 0.37          & 0.36          & 0.28                   & 0.28           \\
\hline
\end{tabular}

==> backup_table.tex <==
\begin{tabular}{ccccccccccc} 
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{DATASET}}}                  & \multicolumn{10}{c}{\textbf{TEAM / BASELINE}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ 
\cline{2-11}
\multicolumn{1}{c|}{}                                                   & \textbf{MoRiHa}                                                                                              & \textbf{neptune}                                                                                             & \textbf{AIpert}                                                                                              & \begin{tabular}[c]{@{}c@{}}\textbf{}\\\textbf{DDQN }\\\textbf{}\end{tabular}                                 & \begin{tabular}[c]{@{}c@{}}\textbf{automl-}\\\textbf{ freiburg}\end{tabular}                                 & \begin{tabular}[c]{@{}c@{}}\textbf{}\\\textbf{BOS}\\\textbf{}\end{tabular}                                   & \begin{tabular}[c]{@{}c@{}}\textbf{}\\\textbf{FT}\\\textbf{}\end{tabular}                                    & \begin{tabular}[c]{@{}c@{}}\textbf{automl-}\\\textbf{hannover}\end{tabular}                                  & \begin{tabular}[c]{@{}c@{}}\textbf{}\\\textbf{AR}\\\textbf{}\end{tabular}                                    & \begin{tabular}[c]{@{}c@{}}\textbf{}\\\textbf{RS}\\\textbf{\textbf{}}\end{tabular}       \\ 
\hline
adult                                                                   & \textbf{0.81}                                                                                                & 0.79                                                                                                         & 0.79                                                                                                         & 0.78                                                                                                         & 0.66                                                                                                         & 0.72                                                                                                         & 0.7                                                                                                          & 0.62                                                                                                         & 0.27                                                                                                         & 0.21                                                                                     \\
albert                                                                  & \textbf{0.32}                                                                                                & 0.3                                                                                                          & 0.29                                                                                                         & 0.29                                                                                                         & 0.3                                                                                                          & 0.24                                                                                                         & 0.24                                                                                                         & 0.22                                                                                                         & 0.2                                                                                                          & 0.05                                                                                     \\
alexis                                                                  & 0.18                                                                                                         & \textbf{0.46}                                                                                                & 0.41                                                                                                         & 0.11                                                                                                         & 0.12                                                                                                         & 0.22                                                                                                         & 0.2                                                                                                          & 0.24                                                                                                         & 0.37                                                                                                         & 0.02                                                                                     \\
arturo                                                                  & \textbf{0.71}                                                                                                & 0.67                                                                                                         & 0.68                                                                                                         & 0.67                                                                                                         & 0.67                                                                                                         & 0.55                                                                                                         & 0.55                                                                                                         & 0.33                                                                                                         & 0.38                                                                                                         & 0.02                                                                                     \\
cadata                                                                  & 0.75                                                                                                         & 0.68                                                                                                         & \textbf{0.77}                                                                                                & 0.54                                                                                                         & 0.73                                                                                                         & 0.7                                                                                                          & 0.68                                                                                                         & 0.74                                                                                                         & 0.26                                                                                                         & 0.01                                                                                     \\
carlo                                                                   & 0.0                                                                                                          & \textbf{0.16}                                                                                                & 0.14                                                                                                         & 0.03                                                                                                         & 0.09                                                                                                         & 0.08                                                                                                         & 0.07                                                                                                         & 0.08                                                                                                         & 0.14                                                                                                         & 0.01                                                                                     \\
christine                                                               & 0.39                                                                                                         & \textbf{0.44}                                                                                                & 0.43                                                                                                         & 0.43                                                                                                         & \textbf{0.44}                                                                                                & 0.35                                                                                                         & 0.34                                                                                                         & 0.38                                                                                                         & 0.33                                                                                                         & 0.01                                                                                     \\
digits                                                                  & 0.74                                                                                                         & \textbf{0.84}                                                                                                & 0.83                                                                                                         & \textbf{0.84}                                                                                                & 0.8                                                                                                          & 0.73                                                                                                         & 0.71                                                                                                         & 0.5                                                                                                          & 0.43                                                                                                         & 0.16                                                                                     \\
dilbert                                                                 & 0.67                                                                                                         & 0.72                                                                                                         & 0.73                                                                                                         & \textbf{0.75}                                                                                                & 0.45                                                                                                         & 0.61                                                                                                         & 0.59                                                                                                         & 0.43                                                                                                         & 0.25                                                                                                         & 0.07                                                                                     \\
dionis                                                                  & \textbf{0.52}                                                                                                & 0.4                                                                                                          & 0.36                                                                                                         & 0.4                                                                                                          & \textbf{0.52}                                                                                                & 0.41                                                                                                         & 0.45                                                                                                         & 0.46                                                                                                         & 0.0                                                                                                          & 0.0                                                                                      \\
dorothea                                                                & 0.83                                                                                                         & \textbf{0.84}                                                                                                & 0.82                                                                                                         & 0.67                                                                                                         & 0.71                                                                                                         & 0.78                                                                                                         & 0.77                                                                                                         & 0.28                                                                                                         & 0.0                                                                                                          & 0.05                                                                                     \\
evita                                                                   & 0.54                                                                                                         & \textbf{0.55}                                                                                                & 0.51                                                                                                         & 0.53                                                                                                         & 0.53                                                                                                         & 0.44                                                                                                         & 0.42                                                                                                         & 0.44                                                                                                         & 0.44                                                                                                         & 0.0                                                                                      \\
fabert                                                                  & \textbf{0.23}                                                                                                & 0.2                                                                                                          & 0.2                                                                                                          & 0.16                                                                                                         & 0.2                                                                                                          & 0.17                                                                                                         & 0.16                                                                                                         & 0.13                                                                                                         & 0.11                                                                                                         & 0.07                                                                                     \\
flora                                                                   & 0.26                                                                                                         & 0.25                                                                                                         & 0.19                                                                                                         & 0.22                                                                                                         & \textbf{0.30}                                                                                                & 0.07                                                                                                         & 0.09                                                                                                         & 0.23                                                                                                         & 0.25                                                                                                         & 0.03                                                                                     \\
grigoris                                                                & 0.05                                                                                                         & \textbf{0.07}                                                                                                & 0.0                                                                                                          & 0.0                                                                                                          & 0.0                                                                                                          & 0.0                                                                                                          & 0.0                                                                                                          & 0.01                                                                                                         & 0.0                                                                                                          & 0.0                                                                                      \\
helena                                                                  & \textbf{0.13}                                                                                                & 0.1                                                                                                          & 0.11                                                                                                         & 0.12                                                                                                         & 0.05                                                                                                         & 0.07                                                                                                         & 0.07                                                                                                         & 0.04                                                                                                         & 0.0                                                                                                          & 0.02                                                                                     \\
jannis                                                                  & \textbf{0.35}                                                                                                & 0.34                                                                                                         & 0.33                                                                                                         & 0.31                                                                                                         & 0.34                                                                                                         & 0.27                                                                                                         & 0.26                                                                                                         & 0.24                                                                                                         & 0.23                                                                                                         & 0.0                                                                                      \\
jasmine                                                                 & \textbf{0.62}                                                                                                & \textbf{0.62}                                                                                                & 0.6                                                                                                          & 0.61                                                                                                         & \textbf{0.62}                                                                                                & 0.5                                                                                                          & 0.48                                                                                                         & \textbf{0.62}                                                                                                & 0.42                                                                                                         & 0.11                                                                                     \\
madeline                                                                & \textbf{0.73}                                                                                                & 0.65                                                                                                         & 0.67                                                                                                         & 0.68                                                                                                         & 0.64                                                                                                         & 0.58                                                                                                         & 0.56                                                                                                         & 0.66                                                                                                         & 0.47                                                                                                         & 0.01                                                                                     \\
marco                                                                   & \textbf{0.32}                                                                                                & 0.17                                                                                                         & 0.19                                                                                                         & 0.12                                                                                                         & 0.0                                                                                                          & 0.0                                                                                                          & 0.0                                                                                                          & 0.06                                                                                                         & 0.0                                                                                                          & 0.02                                                                                     \\
newsgroups                                                              & \textbf{0.23}                                                                                                & 0.15                                                                                                         & 0.06                                                                                                         & 0.1                                                                                                          & 0.08                                                                                                         & 0.06                                                                                                         & 0.06                                                                                                         & 0.07                                                                                                         & 0.05                                                                                                         & 0.0                                                                                      \\
pablo                                                                   & \textbf{0.27}                                                                                                & 0.26                                                                                                         & 0.25                                                                                                         & 0.26                                                                                                         & 0.25                                                                                                         & 0.22                                                                                                         & 0.21                                                                                                         & 0.2                                                                                                          & 0.16                                                                                                         & 0.05                                                                                     \\
philippine                                                              & \textbf{0.53}                                                                                                & 0.52                                                                                                         & 0.48                                                                                                         & 0.51                                                                                                         & 0.52                                                                                                         & 0.43                                                                                                         & 0.41                                                                                                         & 0.51                                                                                                         & 0.4                                                                                                          & 0.06                                                                                     \\
robert                                                                  & \textbf{0.25}                                                                                                & 0.17                                                                                                         & 0.08                                                                                                         & 0.15                                                                                                         & 0.16                                                                                                         & 0.12                                                                                                         & 0.11                                                                                                         & 0.15                                                                                                         & 0.11                                                                                                         & 0.07                                                                                     \\
sylvine                                                                 & \textbf{0.89}                                                                                                & 0.87                                                                                                         & 0.85                                                                                                         & 0.84                                                                                                         & 0.87                                                                                                         & 0.71                                                                                                         & 0.68                                                                                                         & 0.84                                                                                                         & 0.64                                                                                                         & 0.14                                                                                     \\
tania                                                                   & \textbf{0.18}                                                                                                & 0.01                                                                                                         & 0.0                                                                                                          & 0.02                                                                                                         & 0.02                                                                                                         & 0.0                                                                                                          & 0.0                                                                                                          & 0.0                                                                                                          & 0.0                                                                                                          & 0.0                                                                                      \\
volkert                                                                 & \textbf{0.15}                                                                                                & 0.13                                                                                                         & 0.13                                                                                                         & 0.13                                                                                                         & 0.13                                                                                                         & 0.09                                                                                                         & 0.09                                                                                                         & 0.12                                                                                                         & 0.1                                                                                                          & 0.0                                                                                      \\
waldo                                                                   & \textbf{0.52}                                                                                                & 0.5                                                                                                          & 0.5                                                                                                          & 0.49                                                                                                         & 0.49                                                                                                         & 0.4                                                                                                          & 0.4                                                                                                          & 0.38                                                                                                         & 0.33                                                                                                         & 0.19                                                                                     \\
wallis                                                                  & \textbf{0.46}                                                                                                & \textbf{0.46}                                                                                                & 0.38                                                                                                         & 0.4                                                                                                          & 0.34                                                                                                         & 0.35                                                                                                         & 0.35                                                                                                         & 0.38                                                                                                         & 0.33                                                                                                         & 0.01                                                                                     \\
yolanda                                                                 & \textbf{0.24}                                                                                                & 0.21                                                                                                         & 0.21                                                                                                         & 0.2                                                                                                          & 0.21                                                                                                         & 0.18                                                                                                         & 0.18                                                                                                         & 0.18                                                                                                         & 0.14                                                                                                         & 0.03                                                                                     \\ 
\hline
\rowcolor[rgb]{0.929,0.929,0.929} \multicolumn{1}{c|}{\textbf{AVERAGE}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.929,0.929,0.929}}c@{}}0.43\\$\pm$0.25\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.929,0.929,0.929}}c@{}}0.42\\$\pm$0.25\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.929,0.929,0.929}}c@{}}0.40\\$\pm$0.26\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.929,0.929,0.929}}c@{}}0.38\\$\pm$0.26\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.929,0.929,0.929}}c@{}}0.37\\$\pm$0.25\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.929,0.929,0.929}}c@{}}0.34\\$\pm$0.25\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.929,0.929,0.929}}c@{}}0.33\\$\pm$0.24\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.929,0.929,0.929}}c@{}}0.32\\$\pm$0.22\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.929,0.929,0.929}}c@{}}0.23\\$\pm$0.17\end{tabular}} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.929,0.929,0.929}}c@{}}0.05\\$\pm$0.06\end{tabular}  \\
\hline
\end{tabular}
